NGTS-21b: An Inflated Super-Jupiter Orbiting a Metal-poor K dwarf

We report the discovery of NGTS-21b, a massive hot Jupiter orbiting a low-mass star as part of the Next Generation Transit Survey (NGTS). The planet has a mass and radius of $2.36 \pm 0.21$ M$_{\rm J}$, and $1.33 \pm 0.03$ R$_{\rm J}$, and an orbital period of 1.543 days. The host is a K3V ($T_{\rm eff}=4660 \pm 41$, K) metal-poor (${\rm [Fe/H]}=-0.26 \pm 0.07$, dex) dwarf star with a mass and radius of $0.72 \pm 0.04$, M$_{\odot}$,and $0.86 \pm 0.04$, R$_{\odot}$. Its age and rotation period of $10.02^{+3.29}_{-7.30}$, Gyr and $17.88 \pm 0.08$, d respectively, are in accordance with the observed moderately low stellar activity level. When comparing NGTS-21b with currently known transiting hot Jupiters with similar equilibrium temperatures, it is found to have one of the largest measured radii despite its large mass. Inflation-free planetary structure models suggest the planet's atmosphere is inflated by $\sim21\%$, while inflationary models predict a radius consistent with observations, thus pointing to stellar irradiation as the probable origin of NGTS-21b's radius inflation. Additionally, NGTS-21b's bulk density ($1.25 \pm 0.15$, g/cm$^3$) is also amongst the largest within the population of metal-poor giant hosts ([Fe/H] < 0.0), helping to reveal a falling upper boundary in metallicity-planet density parameter space that is in concordance with core accretion formation models. The discovery of rare planetary systems such as NGTS-21 greatly contributes towards better constraints being placed on the formation and evolution mechanisms of massive planets orbiting low-mass stars.

==> NGTS-21b_ An Inflated Super-Jupiter Orbiting a Metal-poor K dwarf/commands.tex <==
% Please use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared
\newcommand{\kepler}{{\it Kepler}}
\newcommand{\corot}{{\it CoRoT}}
\newcommand{\tess}{{\it TESS}}
\newcommand{\plato}{{\it PLATO}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\JWST}{{\it JWST}}
\newcommand{\NGTS}{NGTS}
\newcommand{\TESS}{{\it TESS}}
\newcommand{\gpe}{{GP-EBOP}}
\newcommand{\LSO}{La Silla Observatory}
\newcommand{\PAR}{Paranal Observatory}
\newcommand{\etop}{\emph{top}}
\newcommand{\emid}{\emph{middle}}
\newcommand{\ebot}{\emph{bottom}}
\newcommand{\eleft}{\emph{left}}
\newcommand{\eright}{\emph{right}}
\newcommand{\eTop}{\emph{Top}}
\newcommand{\eMid}{\emph{Middle}}
\newcommand{\eBot}{\emph{Bottom}}
\newcommand{\eLeft}{\emph{Left}}
\newcommand{\eRight}{\emph{Right}}
\newcommand{\btgc}[1]{\textcolor{blue}{[BTG: #1]}}
\newcommand{\jsj}[1]{\textcolor{blue}{[JSJ: #1]}}
% UNITS
\newcommand{\kms}{km\,s$^{-1}$}
\newcommand{\ms}{m\,s$^{-1}$}
\newcommand{\masy}{mas\,y$^{-1}$}
\newcommand{\mpl}{\mbox{M$_{p}$}}
\newcommand{\rpl}{\mbox{R$_{p}$}}
\newcommand{\mstar}{\mbox{M$_{s}$}}
\newcommand{\rstar}{\mbox{R$_{s}$}}
\newcommand{\mjup}{\mbox{M$_{\rm J}$}}
\newcommand{\rjup}{\mbox{R$_{\rm J}$}}
\newcommand{\msun}{\mbox{M$_{\odot}$}}
\newcommand{\rsun}{\mbox{R$_{\odot}$}}
\newcommand{\rearth}{R$_{\oplus}$}
\newcommand{\mearth}{M$_{\oplus}$}
\newcommand{\gccc}{g\,cm$^{-3}$}
\newcommand{\ergscm}{erg\,s$^{-1}$cm$^{-2}$}
\newcommand{\teff}{$T_{\rm eff}$}
\newcommand{\logg}{$\log g$}

==> NGTS-21b_ An Inflated Super-Jupiter Orbiting a Metal-poor K dwarf/properties.tex <==
%Star properties
\newcommand{\Nstar}{NGTS-21}
\newcommand{\Nkamp}{\mbox{$000 \pm000 $}}%Note units m/s.
\newcommand{\Ngamma}{\mbox{$000 \pm000 $}}%Note units km/s
\newcommand{\NRA}{\mbox{$00^{\rmn{h}} 00^{\rmn{m}} 00\fs00$}} %2MASS
\newcommand{\NDec}{\mbox{$-00\degr 00\arcmin 00\farcs 00$}} %2MASS
\newcommand{\NpropRA}{\mbox{$-00.0\pm0.0 $}} %UCAC4 
\newcommand{\NpropDec}{\mbox{$00.0\pm0.0$}} %UCAC4
\newcommand{\Nstarmass}{\mbox{$0.000\,^{+0.000}_{-0.000}$}}
\newcommand{\Nstarradius}{\mbox{$0.000 \pm 0.0000$}}
\newcommand{\Nstardensity}{\mbox{$0.0\,^{+0.0}_{-0.0}$}}
\newcommand{\Nteff}{\mbox{$0000\,^{+00}_{-00}$}}%SED
\newcommand{\Nrotation}{\mbox{00}} %Periodogram
\newcommand{\Nvmag}{\mbox{$0000\pm 0.00$}}%APASS
\newcommand{\Nmetal}{\mbox{0}} %HARPS
\newcommand{\Ndist}{\mbox{$000\,^{+00}_{-00}$}}%SED (pc)
\newcommand{\Nlogg}{\mbox{$0.00 \pm 0.00$}}
\newcommand{\Ngalu}{\mbox{$00.0 \pm 0.0$}}
\newcommand{\Ngalv}{\mbox{$00.0 \pm 0.0$}}
\newcommand{\Ngalw}{\mbox{$00.0 \pm 0.0$}}
\newcommand{\Nvsini}{$0.0$}
%\newcommand{\Nage}{-} 
\newcommand{\NVmag}{$00.000 \pm 0.000$}
\newcommand{\NBmag}{$00.000 \pm 0.000$}
\newcommand{\Nbmag}{$00.000 \pm 0.000$}
\newcommand{\Ngmag}{$00.000 \pm 0.000$}
\newcommand{\Nrmag}{$00.000 \pm 0.000$}
\newcommand{\Nimag}{$00.000 \pm 0.000$}
\newcommand{\NGAIAmag}{$00.000 \pm 0.000$}
\newcommand{\NNmag}{$00.000 \pm 0.000$}
\newcommand{\NJmag}{$00.000 \pm 0.000$}
\newcommand{\NHmag}{$00.000 \pm 0.000$}
\newcommand{\NKmag}{$00.000 \pm 0.000$}
\newcommand{\NWmag}{$00.000 \pm 0.000$}
\newcommand{\NWWmag}{$00.000 \pm 0.000$}

%Planet properties
\newcommand{\Nplanet}{NGTS-21b}
\newcommand{\Nperiod}{\mbox{$1.5433897 \pm 0.0000016$}}
\newcommand{\Nperiodshort}{\mbox{$0.000$}}
\newcommand{\Nduration}{\mbox{$0.00 \pm 0.00$}}%
\newcommand{\Ntc}{\mbox{$000000000.0000000 \pm 0.00000$}}
\newcommand{\Necc}{\mbox{$0.000\,^{+0.000}_{-0.000}$}}% 
\newcommand{\Nmass}{\mbox{$0.000\,^{+0.0000}_{-0.000}$}}%
\newcommand{\Nradius}{\mbox{$0.00\,^{+0.00}_{-0.00}$}}%
\newcommand{\Ndensity}{\mbox{$0.00\,^{+0.00}_{-0.00}$}}%
\newcommand{\NTeq}{\mbox{$000\pm 00$}}%
\newcommand{\Nflux}{\mbox{($0.00\pm0.00) \times 00^{0}$}}%
\newcommand{\Nrratio}{\mbox{$0.000\,^{+0.000}_{-0.000}$}}
\newcommand{\Nau}{\mbox{$0.0000\,^{+0.0000}_{-0.000}$}}%
\newcommand{\Naoverr}{\mbox{$00.0\pm0.0$}}%
\newcommand{\Nsignalsize}{\mbox{$000$}}
\newcommand{\Nimpact}{\mbox{$0.0000\,^{+0.00}_{-0.000}$}}%



